Audio Retrieval with WavText5K and CLAP Training

Audio-Text retrieval takes a natural language query to retrieve relevant audio files in a database. Conversely, Text-Audio retrieval takes an audio file as a query to retrieve relevant natural language descriptions. Most of the literature train retrieval systems with one audio captioning dataset, but evaluating the benefit of training with multiple datasets is underexplored. Moreover, retrieval systems have to learn the alignment between elaborated sentences describing audio content of variable length ranging from a few seconds to several minutes. In this work, we propose a new collection of web audio-text pairs and a new framework for retrieval. First, we provide a new collection of about five thousand web audio-text pairs that we refer to as WavText5K. When used to train our retrieval system, WavText5K improved performance more than other audio captioning datasets. Second, our framework learns to connect language and audio content by using a text encoder, two audio encoders, and a contrastive learning objective. Combining both audio encoders helps to process variable length audio. The two contributions beat state of the art performance for AudioCaps and Clotho on Text-Audio retrieval by a relative 2% and 16%, and Audio-Text retrieval by 6% and 23%.

==> texfiles/abstract.tex <==
\begin{abstract}
\vspace{-0.01in}
% Audio-Text retrieval focuses on using natural language queries for retrieving audio files among a database of audios. Similarly, Text-Audio retrieval uses audio files to retrieve the most appropriate description. 
% The training dataset for audio-retrieval system consists of audio-text pairs, here audio recordings have interaction between different objects, actions, and acoustic scenes, which are coupled with compound natural language descriptions. 
% Such complex scenes make learning the alignment between audio and descriptions difficult and hence audio-retrieval a challenging task.
% In this work we focus on improving audio-retrieval systems and make two contributions.
% First, we introduce the WavText5K dataset containing audio-text pairs with isolated audio events and descriptions. We hypothesize that learning isolated audio events and their description will help audio-retrieval models for learning complex audio scenes and compound descriptions. 
% We experimental show that indeed adding WavText5K to the training data improves audio-retrieval performance. Second, we propose an architecture which uses an objective function based on symmetric cross entropy, and combines the latest advancements in CNN and Transformer models. 
% The two contributions establish SoTA and beat the existing benchmark on AudioCaps and Clotho on Text-Audio retrieval by 2\% and 16\%, and Audio-Text retrieval for by 6\% and 23\% respectively.

Audio-Text retrieval takes a natural language query to retrieve relevant audio files in a database. Conversely, Text-Audio retrieval takes an audio file as a query to retrieve relevant natural language descriptions. Retrieval systems have to learn the alignment between pairs of complex audio content with variable length and their descriptions. Most of the literature train systems with audio captioning datasets containing curated descriptions, but `wild' descriptions from the web are yet underexplored. In this work we propose a new framework for retrieval and a selection of web audio-text pairs. First, our framework learns to connect language and audio content by using a text encoder, two audio encoders, and a contrastive learning objective to learn a joint multimodal space. Combining both audio encoders help to process variable length audio. Second, we provide a selection of five thousand web audio-text pairs that we refer to as WavText5K. When used to train our retrieval system, WavText5K improved performance more than other audio captioning datasets. The two contributions are key to establish state of the art performance for AudioCaps and Clotho on Text-Audio retrieval by a relative 2\% and 16\%, and Audio-Text retrieval by 6\% and 23\% respectively.

\end{abstract}
\begin{keywords}
audio retrieval, text-based retrieval, contrastive learning, metric learning
\end{keywords}
\vspace{-0.15in}

==> texfiles/introduction.tex <==
\vspace{-0.05in}
\section{Introduction}\label{sec:intro}
\vspace{-0.05in}

% \begin{table*}[]
% \footnotesize
% \center
% \begin{tabular}{ccccccccccc} \hline
% Dataset & Source & Language & Dur. (h) & \ \#audios & \#captions & \makecell{max \\ dur.(s)} & \makecell{avg \\ dur.(s)} & \makecell{max \\ #words} & \makecell{avg \\ #words} & Metadata \\ \hline
% AudioCaps \cite{audiocaps} & YouTube & English & 135.01 & 50535 & 55512 & 10.08 & 9.84 & 52 & 8.80 & YouTube meta. \\
% ClothoV2 \cite{clotho} & FreeSound & English  & 37.05 & 5929 & 29645 & 30.00 & 22.50 & 21 & 11.34 & Keywords \\
% Audio Caption \cite{audiocaption}  & Varied  & Chinese  & 10.3 & 3707 & 3707  & N/A & 10.00 & 54 & 11.14 & - \\
% SoundDescs \cite{sounddescs} & BBC & English  & 1060.40  & 32979 & 32979 & 4475.38 & 115.75 & 65 & 15.28 & - \\ 
% MACS \cite{macs} & TUT & English &  11.88 & 3930 & 17275 & 10.88 & 10.88 & 40 & 9.24 & Tags \\ \hline
% WavText5K & \makecell{BigSoundBank \\ SoundBible}  & English & 25.48 & 4525 & 4525 & 2438.65 & 20.27 & 82 & 12.50 & Title, tags \\ \hline
% \end{tabular}
% \caption{\label{table: dataset-description} Audio-text datasets available in literature.\vspace{-0.1in}}
% \end{table*}

\begin{table*}[]
\footnotesize
\center
\begin{tabular}{ccccccccccc} \hline
Dataset & Source & Language & Dur. (h) & \ \#audios & \#captions & \makecell{max \\ dur.(s)} & \makecell{avg \\ dur.(s)} & \makecell{max \\ #words} & \makecell{avg \\ #words} & Caption Type \\ \hline
AudioCaps \cite{audiocaps} & YouTube & English & 135.01 & 50535 & 55512 & 10.08 & 9.84 & 52 & 8.80 & Human annotated \\
ClothoV2 \cite{clotho} & FreeSound & English  & 37.05 & 5929 & 29645 & 30.00 & 22.50 & 21 & 11.34 & Human annotated \\
SoundDescs \cite{sounddescs} & BBC & English  & 1060.40  & 32979 & 32979 & 4475.38 & 115.75 & 65 & 15.28 & Human annotated \\ 
MACS \cite{macs} & TUT & English &  11.88 & 3930 & 17275 & 10.88 & 10.88 & 40 & 9.24 & Human annotated \\ \hline
WavText5K & \makecell{BigSoundBank \\ SoundBible}  & English & 25.48 & 4525 & 4525 & 2438.65 & 20.27 & 82 & 12.50 & Title, Descriptions \\ \hline
\end{tabular}
\caption{\label{table: dataset-description} Audio-text datasets used in this paper. The first four datasets have curated processes to annotate the captions, whereas WavText5K uses the free-form descriptions provided by the users who upload the audio recording.\vspace{-0.1in}}
\end{table*}

% \textbf{[Audio Retrieval]} 
The text to audio (text-audio) retrieval task consisting of retrieving audio files for a textual query. Conversely, the audio to text (audio-text) retrieval task focuses on retrieving descriptions given an audio file. We will use audio-retrieval to refer to both text-audio and audio-text retrieval in this paper. The audio-retrieval technology has numerous applications in search engines, anomaly detection, audio and video editing. 

% \textbf{[Relevant literature]} 
The early works in audio-retrieval focused on using audio rags or events instead of audio description as the queries \cite{10.1145/1460096.1460115, Ikawa2018AcousticES, earlycrossmodal, elizalde2020never}. With availability of audio captioning and audio-text pair datasets \cite{audiocaps,clotho,sounddescs}, the audio-retrieval task was expanded to include natural language descriptions as queries. Specifically, Koepke et al. \cite{oncescu2021audio} and the DCASE challenge 6B \cite{xie2022dcase} repurposed the audio-captioning dataset AudioCaps \cite{audiocaps} and Clotho \cite{clotho} as benchmark datasets for audio-retrieval. The difficulty of building a high performing audio-retrieval system is made evident from the mAP and recall metrics from the DCASE 2022 6B baseline \cite{xie2022dcase}. Therefore, in this work we focus on audio-retrieval for free-form natural language queries. We hypothesize that learning the alignment between isolated audio events and their descriptions, helps in understanding compound natural language queries and audios. For example, an isolated audio event description for crow is: ``A single crow crying in the middle of the night". This description provides more information than prompts like ``this is a sound of crow" and yet at the same time is focused on one sound event of crow crying. We propose WavText5K dataset which contains such isolated audio-text pairs and show the utility of the dataset for improving audio retrieval performance. 

% usage of free-form language-based queries makes audio-retrieval task more challenging as is evident by the mAP and recall metrics in DCASE 2022 6B baseline \cite{xie2022dcase}. 
The models used for audio retrieval consists of an audio encoder and a text encoder. The audio and text encoder bring the audio and text pairs into a joint embedding space. 
% The objective function consists of distance metric to bring corresponding audio-text pairs closer together and at the same time push different audio-text away in the joint embedding space.
The audio-retrieval literature \cite{sounddescs, mei2022metric, oncescu2021audio} uses variants of metric learning \cite{musgrave2020metric} which force corresponding audio-text pairs to lie closer in the joint embedding space.
% and at the same time push different audio-text away in the joint embedding space.
% The approach for audio retrieval include projecting the audio and text into a learned common multimodal space, followed by a distance metric for comparison between the audio and text embeddings. This multimodal space is generally learned with some variant of metric learning \cite{musgrave2020metric}. 
% The choice of distance metric and type of objective function has strong impact on the performance of the audio-retrieval system \cite{sounddescs, mei2022metric, oncescu2021audio}. 
The existing literature \cite{mei2022metric} trains independent models for each target audio-retrieval dataset. 
% However, recent works  \cite{elizalde2022clap, wav2clip, audioclip} in audio pretraining show that large models can be trained on audio-text pairs which can generalise to different tasks and domains.
However, recent audio-pretraining works  \cite{elizalde2022clap, wav2clip, audioclip} show that large models trained on audio-text pairs can generalise to different tasks and domains.
Particularly, a type of such models called CLAP \cite{elizalde2022clap} learns audio concepts from natural language supervision and achieves SoTA in multiple downstream domains. Therefore, we propose an audio-retrieval architecture based on CLAP training which allows us to train a single model which beats SoTA on both the audio-retrieval benchmarks. The architecture combines the audio transformers \cite{htsat, gong2021ssast} with CNN models \cite{pann} to understand temporally long audio scenes.  
% the ability of CNN based audio models \cite{pann} to understand long temporal audio scenes.  
% \textbf{Propose architecture} Therefore in this work, we answer (b) \textit{``Can we create a generalized architecture that achieves SoTA on multiple downstream audio-retrieval benchmarks?"}

% \textbf{[Dataset contribution]} A strong audio-retrieval model requires understanding of not only the individual audio events, but also compound audio concepts and alignment of those concepts to natural language queries. So in this work we answer the question (a) \textit{``Does learning alignment between simple audio event and descriptions help audio-retrieval for compound queries?"}

% \textbf{[CLAP like models]} To improve performance, the existing literature trains independent models for each target dataset. However, recent literature has shown that a generalized model \cite{elizalde2022clap, wav2clip, audioclip} can be trained on audio-text pairs. Specifically, CLAP \cite{elizalde2022clap} learns audio concepts from natural language supervision and achieves SoTA in both Zero-shot and supervised setting in multiple downstream domains. \textbf{Propose architecture} Therefore in this work, we answer (b) \textit{``Can we create a generalized architecture that achieves SoTA on multiple downstream audio-retrieval benchmarks?"}

% \textbf{[Summary]} In all, we make two contributions in this paper. First, we posit that learning alignment between simple audio event and descriptions helps to match compound audio concepts with a natural language queries. Hence, we curate AudioEventCaps dataset which contains audio-text pairs focusing on simple audio events. We source the dataset via varied sources and collect metadata like description, title, tags etc of the audio files. We empirically show that using AudioEventCaps in training data, improves audio-retrieval performance on the benchmark datasets. We also evaluate how construction of captions has effect on audio retrieval performance. Second, we propose a generalized architecture for audio retrieval. The key elements of the architecture are complementary audio encoders and symmetric cross entropy loss function. The proposed architecture beats existing SoTA on audio retrieval datasets. 

% \textbf{[Summary]} 
In all, we make two contributions in this paper. First, we introduce WavText5K dataset which contains isolated audio scenes and their descriptions. We show how this dataset improves performance on audio-retrieval benchmarks.
% containing compound queries and audio concepts. 
Second, we propose an architecture for audio retrieval based on CLAP training and complementary audio encoders. 
% The key elements of the architecture are complementary audio encoders and symmetric cross entropy loss. 
The proposed architecture beats existing SoTA on audio retrieval benchmarks. 

% we posit that learning alignment between simple audio event and descriptions helps to match compound audio concepts with a natural language queries. Hence, we curate AudioEventCaps dataset which contains audio-text pairs focusing on simple audio events. We source the dataset via varied sources and collect metadata like description, title, tags etc of the audio files. We empirically show that using AudioEventCaps in training data, improves audio-retrieval performance on the benchmark datasets. We also evaluate how construction of captions has effect on audio retrieval performance. Second, we propose a generalized architecture for audio retrieval. The key elements of the architecture are complementary audio encoders and symmetric cross entropy loss function. The proposed architecture beats existing SoTA on audio retrieval datasets. 

==> texfiles/method.tex <==
\section{Method}\label{sec:method}
\vspace{-0.05in}
CLAP is illustrated in Fig~\ref{fig:clap_diagram}. The input is audio and text pairs passed to an audio encoder and a text encoder. Both representations are connected in joint multimodal space with linear projections. The space is learned with the (dis)similarity of audio and text pairs in a batch using contrastive learning. The pretrained encoders with their projection layers can be used to compute audio and text embeddings and enable Zero-Shot Classification. Our method is inspired by the CLIP model~\cite{radford2021learning}.
%The pretrained encoders with their projections can be used to extract the text embeddings from the class labels and the audio embeddings from the testing audios.We computed cosine similarity between the embeddings to perform zero-shot linear classification.

\subsection{Contrastive Language-Audio Pretraining}
\vspace{-0.05in}

Let the processed audio be $X_a$ s.t. $X_a \in \mathbb{R}^{F \times T}$ where $F$ are the number of spectral components (e.g. Mel bins) and $T$ are the number of time bins. Let the text be represented by $X_t$. Each audio-text pair in a batch of $N$ is represented as $\{X_a, X_t\}_i$ where $i \in [0,N]$. For convenience, we dropped the $i$ notation, and henceforth $\{X_a, X_t\}$ will denote a batch of N. 

From the pairs, the audio and text are passed through an audio encoder and a text encoder respectively. Let $f_a(.)$ represent the audio encoder and $f_t(.)$ represent the text encoder. For a batch of N:
\begin{equation}
    \hat{X}_a = f_a(X_a); 
    \hat{X}_t = f_t(X_t)
\end{equation}
where $\hat{X}_a \in \mathbb{R}^{N \times V}$ are the audio representations of dimensionality $V$, and $\hat{X}_t \in \mathbb{R}^{N \times U}$ are the text representations of dimensionality $U$. 

We brought audio and text representations, $\hat{X}_a$ and $\hat{X}_t$, into a joint multimodal space of dimension $d$ by using a learnable linear projection: 
\begin{equation}
    E_a = L_a(X_a);
    E_t = L_t(X_t)
\end{equation}
where $E_a \in \mathbb{R}^{N \times d}$, $E_t \in \mathbb{R}^{N \times d}$, $L_a$ and $L_t$ are the linear projections for audio and text respectively. 

Now that the audio and text embeddings ($E_a$, $E_t$) are comparable, we can measure similarity:
\begin{equation}
    C = \tau*(E_t \cdot E_a^\top)
\end{equation}
where $\tau$ is a temperature parameter to scale the range of logits. The similarity matrix $C \in \mathbb{R}^{N \times N}$ has $N$ correct pairs in the diagonal and $N^2-N$ incorrect pairs in the off-diagonal. 
\begin{equation}
     \mathcal{L} = 0.5 * (\ell_{text}(C) + \ell_{audio}(C))
\end{equation}
where $\ell_{k} = \frac{1}{N}\sum_{i=0}^{N} \log diag (softmax(C))$ along text and audio axis respectively. We used this symmetric cross-entropy loss ($\mathcal{L}$) over the similarity matrix to jointly train the audio encoder and the text encoder along with their linear projections. %\soh{Clarify symmetric cross entropy}

\vspace{-0.05in}
\subsection{Zero-Shot Linear Classification}
\label{sec:method,subsec:zeroshot} 
\vspace{-0.05in}

For Zero-Shot classification, we used CLAP's ability to determine the similarity between audio and text. Let's consider a target dataset with $C$ class labels and $N$ test audios. First, we compute audio embeddings and text embeddings for $N$ audios and $C$ classes using the pretrained encoders and their projection layers. Second, because both the embeddings are in a common space, we compute the cosine similarity between each testing audio and all the class labels. Each audio will have as many logits as class labels. Third, logits are turned into a probability distribution by applying softmax for binary or multiclass and sigmoid for multilabel classification. 
\vspace{-0.15in}
